LS-IQ: Implicit Reward Regularization for Inverse Reinforcement Learning

Recent methods for imitation learning directly learn a $Q$-function using an implicit reward formulation rather than an explicit reward function. However, these methods generally require implicit reward regularization to improve stability and often mistreat absorbing states. Previous works show that a squared norm regularization on the implicit reward function is effective, but do not provide a theoretical analysis of the resulting properties of the algorithms. In this work, we show that using this regularizer under a mixture distribution of the policy and the expert provides a particularly illuminating perspective: the original objective can be understood as squared Bellman error minimization, and the corresponding optimization problem minimizes a bounded $\chi^2$-Divergence between the expert and the mixture distribution. This perspective allows us to address instabilities and properly treat absorbing states. We show that our method, Least Squares Inverse Q-Learning (LS-IQ), outperforms state-of-the-art algorithms, particularly in environments with absorbing states. Finally, we propose to use an inverse dynamics model to learn from observations only. Using this approach, we retain performance in settings where no expert actions are available.

==> old_stuff.tex <==
% \citet{Ho2016} introduced adversarial imitation learning by proposing to apply \gls{gans} to Markov decision processes. They related their method, \gls{gail}, to maximum entropy inverse reinforcement learning~\citep{ziebart_phd} and showed that it minimizes the Jensen-Shannon divergence to the expert distribution. \citet{ghasemipour2020} generalized this procedure to general $f$-divergences, based on the generalization of \gls{gans} to $f$-GANs~\citep{nowozin2016}. $f$-divergences are a broad family of divergences that are parameterized by a convex function $f$ and include, among others, the Jensen-Shannon divergence, forward and reverse Kullback-Leibler divergence, the squared Hellinger distance and, of particular interest for this work, the Pearson $\chi^2$ divergence. The $\chi^2$ divergence was proposed for improving the training stability for \gls{gans} \citep{mao2017} and for adversarial imitation learning~\citep{peng2021}. The aforementioned methods require online interactions with the environment to estimate the density ratio of state distributions of policy and expert, which is required for computing the reward function needed to improve the current policy. \citet{kostrikov2019} improved the sample efficiency of \gls{ail} by using a replay buffer for off-policy updates for policy and discriminator. They justified their approach based on importance sampling, but proposed to ignore the importance weights for practical implementations to remove errors caused by the noisy estimates. \citet{kostrikov2019} also pointed out the problem of reward bias, which is a common problem among the aforementioned imitation learning methods. Namely, by not training the density-ratio for absorbing states, \gls{ail} methods implicitly assign a reward of zero to these states, which may lead to survival or termination biases, depending on the chosen divergence. 


% In order to avoid noisy estimates of importance weights for more sample efficient off-policy imitation learning, \citet{kostrikov2020} introduced recent advances from offline policy evaluation~\citep{nachum2019} to the imitation learning setting. Their method, ValueDice, minimizes the reverse Kullback-Leibler divergence to the expert distribution based on its Donsker-Varadhan representation. By using a change of variable, that can also be considered as an inverse Bellman operator~\citep{garg2021}, they express the adversarial reward function in terms of its Q-function for the current policy. The resulting objective can be minimized offline because the expected reward of the agent can be decreased by directly minimizing its value function for the initial states, without requiring policy roll-outs to estimate its induced state-action distribution. Furthermore, by directly learning the Q-function, policy improvement can be performed directly, dropping the policy evaluation step that is common in actor-critic reinforcement learning. Whereas their policy optimization was still based on an adversarial optimization problem, \citet{arenz2020} derived a non-adversarial formulation based on trust-region updates on the policy. Their method, O-NAIL, used a standard soft actor-critic~\citep{sac} update for policy improvement. A similar algorithm for minimizing the reverse KL divergence---but without the need of trust-region updates---was derived by~\citet{garg2021} based on implicit reward regularization. However, they also considered different divergences for different choices of the regularizer, and their main algorithm, \gls{iq}, uses a squared penalty and minimizes the $\chi^2$ divergence, which empirically performs better than the reverse KL divergence. \citet{swamy2021} provide a unifying perspective on aforementioned imitation learning, categorizing them into moment-matching methods, that either match reward of Q-function moments. They also introduce a method, ADRIL, that is related to our method by assigning fixed rewards to expert and policy transition. Using fixed, binary reward functions for imitation learning was originally proposed by \citet{reddy2020} and can be derived from a regularized behavioral cloning objective.

% Our work also considers the problem of imitation learning from observations~\citep{torabi2019_Survey}, which assumes that only the expert's states but not their actions are observed. While the general imitation learning framework based on $f$-GANs can be straightforwardly extended to this problem setting~\citep{arenz2020}, \citet{torabi2019_GaifO} proposed to train the discriminator of GAIL based on state-transitions rather than individual states, which can improve performance by matching the expert's distribution over transitions. Furthermore, some explicit reward methods (e.g. AIRL~\citep{fu2018}) and most implicit reward methods assume action observations and are, thus, not directly applicable. \todo{reminder: Dave rephrase this after moving the end to the section}



% since:
% \begin{equation}
% \argmax_{Q\in\Omega}\bar{\mathcal{J}}(Q, \pi_Q) = \argmin_{Q\in\Omega} \Lls (Q, \pi_Q)    \, .
% \end{equation}

% The hard objective in \gls{rl} is:
% {\small
% \begin{align}
%     J(\pi) =& \mathbb{E}_{\substack{s_0 \sim \iota_0 \\ a_t \sim \pi \\s_{t+1}\sim P}} \left[ \sum_{t=0}^{\infty} \gamma^t r_{t}\right] \\
%     =& \mathbb{E}_{\iota_{0}} \left[V^\pi(s_0)\right]
% \end{align}}
% The soft \gls{rl} objective is given by: 
% {\small
% \begin{align}
%     \tilde{J}(\pi) =& \mathbb{E}_{\substack{s_0 \sim \iota_0 \\ a_t \sim \pi \\s_{t+1}\sim P}}  \left[ \sum_{t=0}^{\infty} \gamma^t r_{t} +  \gamma^t \alpha \mathcal{H}(\pi(.|s_t))\right]\\
%     =& \mathbb{E}_{\substack{s_0 \sim \iota_0 \\ a_t \sim \pi \\s_{t+1}\sim P}}  \left[ \sum_{t=0}^{\infty} \gamma^t r_{t} + \gamma^t \alpha \mathbb{E}_\pi [-\log(\pi(.|s_t)]\right] \\
% \end{align}}

% with the occupancy metric $\rho_\pi(s,a) = \pi(a|s) \sum_{t=0}^\infty \gamma^t P(s_t=s | \pi)$ we can write:
% {\small
% \begin{align}
%     \phantom{\tilde{J}(\pi))}=& \mathbb{E}_{\rho_\pi}  \left[ r(s,a) + \alpha \mathbb{E}_\pi [-\log(\pi(.|s_t)]\right] \\
%     =& \mathbb{E}_{\rho_\pi}  \left[ r(s,a) \right] +  \mathbb{E}_{\rho_\pi}  \left[ \alpha \mathbb{E}_\pi [-\log(\pi(.|s_t)]\right]  \\
%     =& \mathbb{E}_{\iota_{0}} \left[V^\pi(s_0)\right] + \mathbb{E}_{\iota_{0}} \left[H^\pi(s_0)\right]  \\
%     =&  J(\pi) + H(\pi)
% \end{align}}

% We can define multiple $Q$ functions. Starting with he conventional hard $Q$ function:
% {\small
% \begin{align}
% Q^\pi(s,a) =& r(s,a) + \gamma \mathbb{E}_P[V^\pi(s')] \\
% =& r(s,a) + \gamma \mathbb{E}_{\substack{P\\\pi}}[Q^\pi(s', \hat{a})] 
% \end{align}}
% and then the $H$-function:
% {\small
% \begin{align}
% H^\pi(s) =& \mathbb{E}_{\pi}[- \alpha  \log(\pi(a|s)) + \gamma \mathbb{E}_P[H^\pi(s')]]
% \\
%  =& \mathbb{E}_{\pi}[- \alpha  \log(\pi(a|s))]  + \gamma \mathbb{E}_{\pi}\left[ \mathbb{E}_P[H^\pi(s')]\right] \\
% \end{align}}
% %
% leading to the soft $Q$-function:
% %
% {\small
% \begin{align}
% \tilde{Q}^\pi(s_i,a_i) =& r(s_i,a_i) + \gamma \mathbb{E}_P[\tilde{V}^\pi(s')] \\
% =& r(s_i,a_i) + \gamma \mathbb{E}_{\substack{P\\\pi}}[\tilde{Q}^\pi(s', a') - \alpha \log(\pi(a'|s'))] \\
% =& r(s_i,a_i) + \gamma \mathbb{E}_{\substack{P\\\pi}}[
%  r(s',a') + \gamma \mathbb{E}_P[\tilde{V}^\pi(s'')]
% - \alpha \log(\pi(a'|s'))] \\
% =& r(s_i,a_i) + \gamma \mathbb{E}_{\substack{P\\\pi}}[
%  r(s',a') + \gamma \mathbb{E}_{\substack{P \\\pi}}[\tilde{Q}^\pi(s'', a'') - \alpha \log(\pi(a''|s''))]
% - \alpha \log(\pi(a'|s'))]
% \end{align}}
% Rearranging the terms yields:
% {\small
% \begin{align}
% =&\mathbb{E}_{\substack{P\\\pi}}[ \mathbb{E}_{\substack{P\\\pi}}[r(s_i,a_i) + \gamma 
%  r(s',a') + \gamma^2 \tilde{Q}^\pi(s'', a'') - \gamma\alpha \log(\pi(a''|s''))
% - \gamma^2\alpha \log(\pi(a'|s'))]]
% \\
% =& Q^\pi(s_i,a_i) + \gamma \mathbb{E}_{\substack{P}}[ H^\pi(s')]
% \end{align}}


% \begin{lemma}\label{lemma:bound_maximization}
% Let $\bar{r}$ be a scalar value and let $\bar{Q} = \dfrac{\bar{r}}{1-\gamma}$. Then, the following inequality holds:
% \begin{equation}
%     \mathbb{E}_{\mu_E}\left[ \left(r(s,a) - \bar{r}\right)^2\right]\geq (1-\gamma)^2 \left(\mathbb{E}_{\mu_0,\pi^E}\left[ Q^{\pi_E}(s,a) - \bar{Q} \right]\right)^2
%     \label{eq:bound_maximization}
% \end{equation}
% \end{lemma}

% \begin{proof_lemma}{\ref{lemma:bound_maximization}}
% Using Jensen's inequality on the left hand side:
% \begin{equation*}
%     \mathbb{E}_{\mu_E}\left[ \left(r(s,a) - \bar{r}\right)^2\right]\geq  \left(\mathbb{E}_{\mu_E}\left[ r(s,a) - \bar{r}\right]\right)^2
% \end{equation*}

% We can now rewrite the right hand side as follows:
% \begin{align*}
%     \left(\mathbb{E}_{\mu_E}\left[ r(s,a) - \bar{r}\right]\right)^2 &= \dfrac{(1-\gamma)^2}{(1-\gamma)^2}\left(\mathbb{E}_{\mu_E}\left[ r(s,a) - \bar{r}\right]\right)^2 \\
%     & = (1-\gamma)^2 \left(\mathbb{E}_{\mu_E}\left[ \dfrac{r(s,a)}{(1-\gamma)} - \dfrac{\bar{r}}{(1-\gamma)}\right]\right)^2 \\
%     & = (1-\gamma)^2 \left(\mathbb{E}_{\mu_E}\left[ \dfrac{r(s,a)}{(1-\gamma)} - \bar{Q}\right]\right)^2 \\
%      & = (1-\gamma)^2 \left(\dfrac{\mathbb{E}_{\mu_E}\left[ r(s,a)\right] }{(1-\gamma)}- \bar{Q}\right)^2
% \end{align*}

% By definition
% \begin{equation*}
%  \mathcal{J}(\pi_E) = \dfrac{\mathbb{E}_{\mu_E}\left[ r(s,a)\right]}{1-\gamma} = \mathbb{E}_{\mu_0,\pi_E} \left[ Q(s,a) \right] 
% \end{equation*}

% By using the last equation, and rearranging the left hand side of the inequality we get:
% \begin{equation*}
% \mathbb{E}_{\mu_E}\left[ \left(r(s,a) - \bar{r}\right)^2\right]\geq (1-\gamma)^2 \left(\mathbb{E}_{\mu_0,\pi^E}\left[ Q^{\pi_E}(s,a) - \bar{Q} \right]\right)^2
% \end{equation*}
% \end{proof_lemma}


